Back to the Basics on Predicting Transfer Performance

In the evolving landscape of deep learning, selecting the best pre-trained models from a growing number of choices is a challenge. Transferability scorers propose alleviating this scenario, but their recent proliferation, ironically, poses the challenge of their own assessment. In this work, we propose both robust benchmark guidelines for transferability scorers, and a well-founded technique to combine multiple scorers, which we show consistently improves their results. We extensively evaluate 13 scorers from literature across 11 datasets, comprising generalist, fine-grained, and medical imaging datasets. We show that few scorers match the predictive performance of the simple raw metric of models on ImageNet, and that all predictors suffer on medical datasets. Our results highlight the potential of combining different information sources for reliably predicting transferability across varied domains.

==> 05-table-results.tex <==
\begin{table*}[!ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{clcccccccccccc}
    \toprule
         &Scorer  &Caltech101  &DTD  &OxfordPets  &SUN397  &VOC2007  &Aircraft  &Flowers102  &StanfordCars  &BrainTumor & BreakHis  & ISIC2019 & Avg \\ \toprule
        \multirow{14}{*}{\begin{turn}{90}Linear\end{turn}} &ImageNet  &0.709  &0.636  &\cellcolor{brown}0.782  &\cellcolor{brown} 0.697  &0.648  &0.673  &\cellcolor{brown} 0.515  &0.600  &\cellcolor{brown} 0.673 & 0.467  & \cellcolor{lightgray} 0.552 & \cellcolor{lightgray} 0.632 \\ 
        ~ &H-Score~\cite{hscore}  &0.297  &0.006  &0.127  &0.321  &0.115  &-0.406  &-0.455  &-0.079  &0.236 & 0.467  & \cellcolor{lightgray}0.552 & 0.107 \\ 
        ~ &NCE~\cite{nce}  &0.709  &\cellcolor{lightgray}0.745  &0.721  &0.624  &0.345  &0.079  &-0.273  &0.394  &-0.709 & 0.103  & -0.673 & 0.188 \\ 
        ~ &LEEP~\cite{leep}  &0.733  &0.600  &\cellcolor{brown}0.782  &0.539  &0.842  &0.079  &0.333  &0.273  &-0.188 & 0.224  & -0.055 & 0.378 \\ 
        ~ &$\mathcal{N}$LEEP~\cite{nleep}  &0.370  &0.479  &0.721  &0.564  &0.867  &0.333  &0.442  &0.564  &0.236 & -0.358  & -0.491 & 0.339 \\ 
        ~ &PARC~\cite{parc}  &0.709  &\cellcolor{yellow!75}0.855  &0.455  &0.382  &0.770  &\cellcolor{brown}0.855  &0.418  &0.345  &0.248 & 0.406  & 0.079 & 0.502 \\ 
        ~ &Reg. H-Score~\cite{reghscore}  &0.103  &-0.006  &0.018  &0.188  &-0.091  &-0.248  &-0.394  &-0.248  &-0.273 & 0.297  & -0.188 & -0.077 \\ 
        ~ &SFDA~\cite{sfda}  &0.394  &0.382  &0.321  &0.430  &0.273  &0.455  &0.512  &0.455  &0.200 & 0.491  & 0.042 & 0.360 \\ 
        ~ &LogME~\cite{logme}  &0.345  &0.576  &0.358  &0.527  &0.648  &0.321  &0.030  &0.261  &0.127 & \cellcolor{lightgray}0.745  & \cellcolor{brown}0.406 & 0.395 \\ 
        ~ &GBC~\cite{gbc}  &\cellcolor{yellow!75}0.939  &\cellcolor{brown}0.685  &0.479  &0.661  &\cellcolor{brown}0.879  &\cellcolor{lightgray}0.867  &0.455  &0.370  &0.394 & -0.176  & -0.200 & 0.487 \\ 
        ~ &PACTran~\cite{pactran}  &0.624  &0.564  &0.406  &\cellcolor{lightgray}0.709  &0.358  &0.782  &0.491  &\cellcolor{brown}0.842  &\cellcolor{yellow!75}0.903 & \cellcolor{yellow!75}0.758  & 0.188 & \cellcolor{brown}0.602 \\ 
        ~ &ETran~\cite{etran}  &\cellcolor{lightgray}0.855  &0.576  &\cellcolor{yellow!75}0.879  &\cellcolor{yellow!75}0.867  &\cellcolor{yellow!75}0.915  &0.806  &\cellcolor{lightgray}0.721  &\cellcolor{yellow!75}0.915  &\cellcolor{lightgray}0.842 & 0.297  & \cellcolor{yellow!75}0.685 & \cellcolor{yellow!75}\textbf{0.760} \\ 
        ~ &NCTI~\cite{ncti}  &\cellcolor{brown}0.842  &\cellcolor{yellow!75}0.855  &\cellcolor{lightgray}0.830  &0.673  &\cellcolor{lightgray}0.903  &\cellcolor{yellow!75}0.964  &\cellcolor{yellow!75}0.818  &\cellcolor{lightgray}0.891  &0.661 & \cellcolor{brown}0.709  & 0.212 & \cellcolor{yellow!75}\textbf{0.760} \\ 
        ~ &TMI~\cite{tmi}  &0.539  &0.515  &0.418  &0.612  &0.503  &0.212  &0.418  &0.503  &0.370 & \cellcolor{brown}0.709  & 0.224 & 0.457 \\
        \midrule
        \multirow{14}{*}{\begin{turn}{90}Fine-tune\end{turn}}  &ImageNet  &\cellcolor{brown}0.879  &\cellcolor{brown}0.758  &\cellcolor{yellow!75}0.915  &\cellcolor{brown}0.903  &\cellcolor{brown}0.867  &0.794  &\cellcolor{lightgray}0.673  &\cellcolor{brown}0.794  &0.406 & \cellcolor{lightgray}0.588  & \cellcolor{lightgray}0.661 & \cellcolor{lightgray}0.749 \\ 
        ~ &H-Score~\cite{hscore}  &0.309  &0.164  &0.333  &0.685  &0.406  &-0.273  &-0.297  &0.200  &-0.139 & 0.370  & 0.406 & 0.197 \\ 
        ~ &NCE~\cite{nce}  &0.855  &0.709  &\cellcolor{lightgray}0.855  &\cellcolor{lightgray}0.952  &0.636  &0.006  &-0.261  &0.612  &-0.200 & -0.212  & -0.152 & 0.345 \\ 
        ~ &LEEP~\cite{leep}  &0.733  &0.624  &\cellcolor{brown}0.794  &0.830  &0.842  &0.091  &0.394  &0.527  &0.006 & 0.030  & 0.370 & 0.476 \\ 
        ~ &$\mathcal{N}$LEEP~\cite{nleep}  &0.721  &0.527  &\cellcolor{brown}0.794  &0.842  &0.818  &0.127  &0.552  &\cellcolor{brown}0.794  &-0.333 & 0.382  & -0.236 & 0.453 \\ 
        ~ &PARC~\cite{parc}  &\cellcolor{yellow!75}0.939  &\cellcolor{lightgray}0.855  &0.576  &0.806  &0.721  &\cellcolor{lightgray}0.842  &0.576  &0.576  &-0.442 & \cellcolor{brown}0.503  & -0.067 & 0.535 \\ 
        ~ &Reg. H-Score~\cite{reghscore}  &0.309  &0.091  &0.261  &0.552  &0.236  &-0.273  &-0.067  &-0.042  &-0.491 & -0.309  & -0.370 & -0.009 \\ 
        ~ &SFDA~\cite{sfda}  &0.345  &0.491  &0.455  &0.758  &0.539  &0.515  &\cellcolor{brown}0.649  &0.612  &0.127 & -0.091  & -0.164 & 0.385 \\ 
        ~ &LogME~\cite{logme}  &0.770  &0.624  &0.564  &0.855  &0.794  &0.285  &0.297  &0.479  &-0.248 & 0.212  & \cellcolor{brown}0.576 & 0.473 \\ 
        ~ &GBC~\cite{gbc}  &0.782  &0.697  &0.673  &0.842  &\cellcolor{brown}0.855  &\cellcolor{yellow!75}0.939  &0.564  &0.588  &-0.127 & 0.152  & -0.067 & 0.536 \\ 
        ~ &PACTran~\cite{pactran}  &0.539  &0.685  &0.515  &0.358  &0.394  &0.758  &0.648  &\cellcolor{lightgray}0.879  &\cellcolor{yellow!75}0.721 & 0.248  & 0.115 & 0.533 \\ 
        ~ &ETran~\cite{etran}  &\cellcolor{lightgray}0.903  &0.624  &0.770  &0.491  &\cellcolor{lightgray}0.879  &0.782  &0.600  &\cellcolor{yellow!75}0.891  &\cellcolor{yellow!75}0.733 & \cellcolor{yellow!75}0.842  & 0.661 & \cellcolor{brown}0.743 \\ 
        ~ &NCTI~\cite{ncti}  &\cellcolor{brown}0.879  &\cellcolor{yellow!75}0.879  &\cellcolor{yellow!75}0.915  &\cellcolor{yellow!75}0.976  &\cellcolor{yellow!75}0.939  &\cellcolor{yellow!75}0.939  &\cellcolor{yellow!75}0.806  &\cellcolor{lightgray}0.879  &0.273 & 0.248  & \cellcolor{yellow!75}0.770 & \cellcolor{yellow!75}\textbf{0.776} \\ 
        ~ &TMI~\cite{tmi}  &0.394  &0.564  &0.430  &0.345  &0.552  &0.200  &0.467  &0.636  &\cellcolor{brown}0.515 & 0.115  & 0.261 & 0.407 \\ 
         
        \bottomrule
    \end{tabular}
    }
    \caption{Spearman's correlation index considering all transferability scorers (rows) and datasets (columns) on linear probing and fine-tuning settings. The top half of the table shows results from linear transfer, and the bottom half shows the results when these models are fine-tuned. Observe that ImageNet baseline is competitive in both scenarios, being ranked as the second best scorer in average. We highlight the top-3 best correlation indexes on each column according to their rank: 1st (\crule[yellow!75]{0.4cm}{0.2cm}), 2nd (\crule[lightgray]{0.4cm}{0.2cm}), and 3rd (\crule[brown]{0.4cm}{0.2cm}).   }
    \label{tab:results_linear_ft}
\end{table*}

==> 99-table-datasets.tex <==
% generalist, natural, artifacts, medical
\begin{table}[h!]
  \centering
  \tiny
  % \resizebox{\columnwidth}{!}{%
  \begin{tabular}{>{\raggedright\arraybackslash}p{2.1cm}>{\raggedright\arraybackslash}p{1.1cm}>{\raggedright\arraybackslash}p{0.2cm}>{\raggedright\arraybackslash}p{1cm}>{\raggedright\arraybackslash}p{1.5cm}}
    \toprule
    Dataset & Size (train/test) & Cls. & Target task & Category \\
    \midrule
    Caltech-101 (Cal-101) & 3,060/6,084 & 102 & Objects & Generalist \\    SUN397 & 19,850/19,850 & 397 & Scenes & Generalist \\
    VOC2007 & 5,011/4,952 & 20 & Objects & Generalist \\
    
    Oxford Flowers (Ox.Flowers) & 2,040/6,149 & 102 & Flowers & Generalist/Natural \\
    Oxford-IIIT Pets (Ox.Pets) & 3,680/3,369 & 37 & Animals & Generalist/Natural \\
    FGVC-Aircraft (Aircraft) & 6,667/3,333 & 100 & Aircraft & Generalist/Artifacts \\
    DTD & 3,760/1,880 & 47 & Textures & Generalist/Artifacts \\
    StanfordCars (Stan.Cars) & 8,144/8,041 & 196 & Cars & Generalist/Natural \\
    BrainTumor & 2,870/394 & 4 & Brain MRI & Medical \\
    BreakHis & 6,327/1,582 & 2 & Histopathology & Medical \\
    ISIC 2019 & 16,736/3,863 & 2 & Skin lesion & Medical\\
    \bottomrule
  \end{tabular}
  % }
  \caption{Dataset information. Cls.: Number of classes.}
  \label{tab:datasets}
\end{table}


